FED-HARGPT: A Hybrid Centralized-Federated Approach of a Transformer-based Architecture for Human Context Recognition

The study explores a hybrid centralized-federated approach for Human Activity Recognition (HAR) using a Transformer-based architecture. With the increasing ubiquity of edge devices, such as smartphones and wearables, a significant amount of private data from wearable and inertial sensors is generated, facilitating discreet monitoring of human activities, including resting, sleeping, and walking. This research focuses on deploying HAR technologies using mobile sensor data and leveraging Federated Learning within the Flower framework to evaluate the training of a federated model derived from a centralized baseline. The experimental results demonstrate the effectiveness of the proposed hybrid approach in improving the accuracy and robustness of HAR models while preserving data privacy in a non-IID data scenario. The federated learning setup demonstrated comparable performance to centralized models, highlighting the potential of federated learning to strike a balance between data privacy and model performance in real-world applications.

==> 6-future.tex <==
\section{Future Works}
\label{sec:sec6}

{\color{red}
As future works we expect to design and run experiments considering real Android devices or Android device farms to be able to measure parameters on those specific hardware. We would like to collect network performance metrics in poorly or intermittently available connections and observe how these adversities affect performance. Also, we would like to produce more descriptive labels for future usage with Natural Language Processing (NLP) techniques for further investigation.}
